InfoCon: Concept Discovery with Generative and Discriminative Informativeness

We focus on the self-supervised discovery of manipulation concepts that can be adapted and reassembled to address various robotic tasks. We propose that the decision to conceptualize a physical procedure should not depend on how we name it (semantics) but rather on the significance of the informativeness in its representation regarding the low-level physical state and state changes. We model manipulation concepts (discrete symbols) as generative and discriminative goals and derive metrics that can autonomously link them to meaningful sub-trajectories from noisy, unlabeled demonstrations. Specifically, we employ a trainable codebook containing encodings (concepts) capable of synthesizing the end-state of a sub-trajectory given the current state (generative informativeness). Moreover, the encoding corresponding to a particular sub-trajectory should differentiate the state within and outside it and confidently predict the subsequent action based on the gradient of its discriminative score (discriminative informativeness). These metrics, which do not rely on human annotation, can be seamlessly integrated into a VQ-VAE framework, enabling the partitioning of demonstrations into semantically consistent sub-trajectories, fulfilling the purpose of discovering manipulation concepts and the corresponding sub-goal (key) states. We evaluate the effectiveness of the learned concepts by training policies that utilize them as guidance, demonstrating superior performance compared to other baselines. Additionally, our discovered manipulation concepts compare favorably to human-annotated ones while saving much manual effort.

==> sections/07_ethics.tex <==
\paragraph{Ethics Statement:}
Our research delves into the exploration of potential concepts beyond common semantics. At present, our exploration is centered on the extraction of concepts from basic manipulation tasks, and this will remain our focus. While we are aware of the potential of the algorithm to progress toward understanding more complex concepts, we will proceed with caution, mindful of ethical considerations and the need for responsible control mechanisms.

==> sections/08_reproducibility.tex <==
\paragraph{Reproducibility Statement:}
We provide our implementation details of InfoCon in the appendix (Sec.~\ref{sec:arch_details} and Sec.~\ref{sec:train_detail}, providing details of InfoCon's architecture and training details). 
Our experiments use the state-based environments in ManiSkill2 since the current development of state-based manipulation learning is relatively more mature than vision-based manipulation learning. 
We welcome discussion and advice on better and more stable performance of InfoCon and downstream policies and even further implementation improvement in more practical environments.
